Large Language Models Are Active Critics in NLG Evaluation

The conventional paradigm of using large language models (LLMs) for natural language generation (NLG) evaluation relies on pre-defined task definitions and evaluation criteria, positioning LLMs as "passive critics" that strictly follow developer-provided guidelines. However, human evaluators often apply implicit criteria, and their expectations in practice can vary widely based on specific end-user needs. Consequently, these rigid evaluation methods struggle to adapt to diverse scenarios without extensive prompt customization. To address this, we introduce Active-Critic, a novel LLM-based evaluator that transforms LLMs into "active critics'' capable of adapting to diverse NLG tasks using limited example data. Active-Critic consists of two stages: (1) self-inferring the target NLG task and relevant evaluation criteria, and (2) dynamically optimizing prompts to produce human-aligned scores along with detailed justifications. Our experiments show that Active-Critic can generate nuanced, context-aware evaluation criteria, enabling it to achieve superior alignment with human judgments across multiple tasks.

==> backup.tex <==
%% ========result section=========

\paragraph{Consistency of human judgments.} Table \ref{tab:main-result-orca2} displays the correlation results between unified evaluators and human judgments. According to the average correlation results across diverse NLG evaluation tasks, our approach noticeably outperforms the corresponding prompting-based baselines and state-of-the-art fine-tuning-based evaluators, particularly for the variants built on GPT-4 and ORCA-13B. Comparing \method's performance across two evaluation levels on each LLM, we find that the fine-grained variant consistently achieves closer alignment with human ratings, outperforming the coarse-grained variant by $\sim$2\% in correlation. These findings support our intuition that encouraging LLMs to actively engage in diverse evaluation scenarios by deeply analyzing example data can enhance their ability to capture human-centric assessment nuances per scenario and make more human-aligned judgments. Additionally, forcing the model to think thoroughly about each inferred criterion benefits their decision-making.

\paragraph{Sensitivity to base LLM.} Further looking into the effect of base LLMs on \method, we observe that our approach consistently achieves a noticeable improvement, with an average gain of $\sim$6.8\% correlation over the zero-shot baseline for each base model. These results suggest that our approach can enhance the NLG evaluation capabilities of various LLMs. As expected, \method generally obtains greater enhancements when employing a stronger base LLM. However, it is noteworthy that \method built on Orca2-13B performs comparably to its GPT-4 counterpart on SFRES and OpenMEVA (ROC), indicating that \mj{should add some insights}. Considering the computational cost and evaluator performance, we primarily focus on the ORCA2-based AC-Fine for further analysis.

%we observe that the powerful closed-source LLM, GPT-4, demonstrates strong performance, noticeably outperforming state-of-the-art unified evaluators fine-tuned on LLMs, even in a zero-shot setting. Despite that, the best variants of \method, leveraging both an open-source LLM (Orca2-13B, 0.4677) and a closed-source LLM (GPT-4, 0.5294), achieve higher average correlations with human judgments than this strongest baseline (0.4661) across four NLG tasks. 


% \paragraph{\method outperforms baseline evaluators across four distinct NLG tasks.} Table \ref{tab:main-result-orca2} displays the correlation results between unified evaluators and human judgments on four distinct NLG tasks. Overall, we observe that the coarse and fine variants of \method consistently exhibit a higher correlation with human judgments than baselines across three correlation coefficients in four NLG tasks. The fine-level evaluation generally outperforms the coarse variant. Among three variants, the vanilla \method performs the worst, even with lower average correlation compared to UniEval and ExplainEval. Our observations suggest that while the backbone LLM's (i.e., Orca2-13B) intrinsic knowledge is limited for directly scoring data without task-specific inference, even with prompt optimization using a few examples, our proposed active-critic mechanism can effectively unlock the model's potential to deeply digging into the example data for evaluation. Moreover, this mechanism enhances the model's ability to assess data quality with greater alignment to human judgments. Notably, guiding the model to evaluate each inferred criterion individually leads to better final decisions than asking it to directly provide an overall score.



% \input{tables/00_mian_gpt3.5} 



%While closed-source models (e.g., GPT-4, GPT-3.5) outperform open-source counterparts (e.g., LLaMA3-8B, Orca2-13B), likely due to differences in scale, pretraining data, and optimization, Orca2-13B demonstrates competitive performance. 


% \new{
% \paragraph{ACTIVE-CRITIC generally achieves further improvements with a stronger backbone LLM.} As shown in Table~\ref{tab:main-result-orca2}, GPT-4-based models consistently achieve the best performance in both AC-FINE and AC-COARSE settings, highlighting its superiority as a backbone. While closed-source models (e.g., GPT-4, GPT-3.5) outperform open-source counterparts (e.g., LLaMA3-8B, Orca2-13B), likely due to differences in scale, pretraining data, and optimization, Orca2-13B demonstrates competitive performance. These results indicate that stronger LLMs generally yield better outcomes, but the extent of improvement depends on the dataset and model adaptability.
% }

% the average performance across the four tasks increases as the backbone LLM scales from Orca2-13B to GPT-3.5 and then to GPT-4, improving from 0.4677 to 0.4777, and further to 0.5294 in AC-Fine. This improvement is particularly pronounced in datasets like SummEval and TopicalChat. For example, in SummEval, the Pearson $\gamma$ rises from 0.6301 to 0.6530 and reaches 0.6926. Similarly, in TopicalChat, the Pearson $\gamma$ increases from 0.6023 to 0.6718 and then to 0.7789, showcasing clear gains.
% However, this improvement is not consistent across all datasets. For instance, in SFRES, the performance with GPT-3.5 (0.2833 Spearman $\rho$ and 0.2342 Kendall-Tau $\tau$) and GPT-4 (0.2809 Spearman $\rho$ and 0.2360 Kendall-Tau $\tau$) is similar to or slightly below that of Orca2-13B (0.2834 Spearman $\rho$ and 0.2289 Kendall-Tau $\tau$). Likewise, in OpenMEVA, Orca2-13B outperforms GPT-3.5 on metrics such as Kendall-Tau $\tau$ (0.3209 vs. 0.2981) and Spearman $\rho$ (0.4245 vs. 0.3766). These results suggest that while stronger LLMs generally lead to better performance, the extent of improvement depends on the specific dataset and the model's adaptability.

% \paragraph{\method can achieve further improvements with a stronger backbone LLM.} Comparatively, \method built on GPT-3.5 shows significantly higher correlations with human judgments than the variant built on Orca-13B, indicating that a stronger backbone model enhances the effectiveness of our evaluation protocol. Further comparison with the state-of-the-art GPT-3.5-based baseline reveals that \method consistently outperforms it. As with the Orca-13B-based \method (see Table~\ref{tab:main-result-orca2}), the fine-level variant surpasses the coarse one, further suggesting that multi-criteria scoring and explanations help the backbone LLM conduct a more in-depth analysis of instance quality and make better final decisions.



% % 在文字旁边插入图片
% \begin{wrapfigure}{R}{0.57\textwidth}  % R 表示图片在右侧, L 表示在左侧
% \vspace{-3mm}
%   \centering
%   \includegraphics[width=0.57\textwidth]{figs/effectiveness_of_explanation_Kendall.pdf}  % 设置图片路径与宽度
%   \caption{Comparison of the performance of \method w/ vs. w/o explanations across four NLG tasks. We measure \method's performance by Kendall-Tau correlation (\%). Both coarse-level (AC-Coarse) and fine-level (AC-Fine) variants are investigated.}
%     \label{fig:effectiveness_of_explanation1_compiled}
% \vspace{-3mm}
% \end{wrapfigure}



%As presented in Table~\ref{tab:main-result-gpt}, our Self-Thinking Eval framework also delivers strong performance when using the GPT-3.5 model. The Fine-grained configuration (SRE-Fine) achieved the best results overall, with a Pearson correlation of 0.7152 on TopicalChat and the highest Spearman correlation of 0.6109 on SummEval. 

%As presented in Table~\ref{tab:main-result-gpt}, our Self-Thinking Eval framework also delivers strong performance when using the GPT-3.5 model. The Fine-grained configuration (SRE-Fine) achieved the best results overall, with a Pearson correlation of 0.7152 on TopicalChat and the highest Spearman correlation of 0.6109 on SummEval. SRE-Fine demonstrated consistent superiority. The Coarse-grained configuration (SRE-Coarse), while performing slightly lower than SRE-Fine on most tasks, still achieved competitive results, particularly in the Pearson correlation on SummEval, where it outperformed SRE-Fine. 



%Notably, SRE-Fine demonstrated more stable performance when using GPT-3.5 compared to Orca2-13B. This can be attributed to GPT-3.5's advanced capabilities, which make it more suitable for handling complex optimization tasks like those in fine-grained evaluations. The results indicate that the stronger the LLM used, the better the framework performs, particularly in tasks that require detailed, multi-criteria scoring and explanations.

==> tables/00_main_orca2.tex <==

\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccc|c}
\toprule
~ & \multicolumn{3}{c}{SummEval} & \multicolumn{3}{c}{TopicalChat} & \multicolumn{3}{c}{SFRES} & \multicolumn{3}{c|}{OpenMEVA (ROC)}& \multirow{2}{*}{Average}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}  ~& $\gamma$ & $\rho$ & $\tau$ & $\gamma$ & $\rho$ & $\tau$ & $\gamma$ & $\rho$ & $\tau$ & $\gamma$ & $\rho$ & $\tau$ \\
\midrule

Auto-J & 0.1345 & 0.1457 & 0.1149 & 0.4681 &0.459 & 0.3714 & 0.126 & 0.1022 &0.0809&0.3896&0.3704&0.3065 & 0.2558\\
UniEval & 0.5457 & 0.4914 & 0.3707 & 0.5133 & 0.5448& 0.4134 &0.2894 &0.2499 & 0.1877&0.4501&0.4408&0.3119 &0.4008 \\
GPTScore-src & 0.4043 & 0.3584 & 0.2696 & 0.2313 & 0.2437& 0.1792 &0.2062 &0.121  & 0.1132&0.2283&0.2265&0.1534& 0.2280\\
ExplainEval & 0.5447 & 0.4916 & 0.3999 & 0.5542 & 0.5512 & 0.4476 & 0.1993 & 0.1181 &0.0946 &0.4809&0.4695&0.358&0.3924\\
% TIGERScore & 0.4422 & 0.3681 & 0.3129 & - & -& - &- &-  & - &0.4766&0.4636&0.3533&-&-&-\\

\midrule

\multicolumn{13}{l}{$\textbf{Ours}$} \\

\textsc{AC-Vanilla}& \underline{0.5494} & 0.486 & 0.3964 & 0.4932 &0.4927 & 0.4055 &0.2322 &0.1712  & 0.1328 &0.4023&0.4245 & 0.3209 &0.3756\\

\textsc{AC-Coarse} & 0.5386 & \underline{0.5227} & \underline{0.4156} & \textbf{0.611} & \underline{0.6173}& \textbf{0.4845} &\textbf{0.3094} &\textbf{0.2663}  & \textbf{0.199} &\underline{0.4908} &\underline{0.4962}  & \underline{0.3622}&\underline{0.4428}\\


\textsc{AC-Fine} & \textbf{0.6301} & \textbf{0.5486} & \textbf{0.4299} & \underline{0.6023} & \textbf{0.6214}& \underline{0.4713} &\underline{0.2915}&\underline{0.2501}  & \underline{0.1906} &\textbf{0.5259} &\textbf{0.5363}  & \textbf{0.4109}&\textbf{0.4591}\\




\bottomrule
\end{tabular}
}
\caption{Correlation between LLM-based unified evaluators and human judgments on overall quality per instance across four NLG tasks. All train-free evaluators are built upon Orca2-13B. We compare Pearson ($\gamma$), Spearman ($\rho$) and Kendall-Tau ($\tau$) correlation, respectively. The best performance per indicator is highlighted in bold, and the second-highest results are underlined. We implemented and tested all the methods with p-value $<$ 0.05. %Main results based on Orca2-13B: Pearson ($\gamma$), Spearman ($\rho$) and Kendall-Tau ($\tau$) correlations between different metrics and human judgments of overall quality across four NLG evaluation tasks. We developed three experimental variants: Vanilla, Coarse-grained, and Fine-grained. We systematically investigated the performance variations of each variant under different optimization configurations. In each column, the highest values are highlighted in \textbf{bold}, while the second-highest values are \underline{underlined}. 
}
\label{tab:main-result-orca2} 
\end{table}





% \begin{table}[htbp]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{lcccccccccccc|ccc|c}
% \toprule
% ~ & \multicolumn{3}{c}{SummEval} & \multicolumn{3}{c}{TopicalChat} & \multicolumn{3}{c}{SFRES} & \multicolumn{3}{c}{OpenMEVA}& \multicolumn{4}{c}{Average}\\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-17} ~& $\gamma$ & $\rho$ & $\tau$ & $\gamma$ & $\rho$ & $\tau$ & $\gamma$ & $\rho$ & $\tau$ & $\gamma$ & $\rho$ & $\tau$ & $\gamma$ & $\rho$ & $\tau$& AVE\\
% \midrule
% \multicolumn{13}{l}{$\textbf{Explanation-Based\ Baseline\ (Orca2-13B)}$}  \\
% ExplainEval~\citep{mahmoudi2023exploring} & 0.5746 & 0.5037 & 0.4038 & 0.5788 & 0.5706 & 0.4646 & 0.3068 & 0.2300 &0.1842 &0.4702&0.4611&0.3531&0.4826&0.4414&0.3514&0.4251\\
% \midrule
% \multicolumn{13}{l}{$\textbf{General\ baseline}$}  \\
% Auto-J~\citep{li2023autoj} & 0.1348 & 0.1464 & 0.1155 & 0.4819 &0.475 & 0.3927 & 0.1315 & 0.1053 &0.0869&0.3915&0.3799&0.3101 &0.2849&0.2767&0.2263&0.2626 \\
% UniEval~\citep{zhong2022unieval} & 0.5569 & 0.4739 & 0.3780 & 0.5326 & 0.5769& 0.4363 &0.3247 &0.2791  & 0.2081&0.4488&0.4446&0.3122 & 0.4658& 0.4436&0.3337&0.4144\\
% GPTScore-src~\citep{fu2023gptscore} & 0.4103 & 0.3618 & 0.2721 & 0.2497 & 0.2610& 0.1922 &0.2819 &0.2082  & 0.1618&0.2348&0.2319&0.1645&0.2942&0.2657&0.1977&0.2525 \\
% % TIGERScore & 0.4422 & 0.3681 & 0.3129 & - & -& - &- &-  & - &0.4766&0.4636&0.3533&-&-&-\\
% \midrule
% \multicolumn{13}{l}{$\textbf{Our\ Results\ (Orca2-13B)}$} \\
% \textbf{Vanilla} & 0.5284 & 0.4602 & 0.3689 & 0.5003 &0.5091 & 0.4018 & 0.3166 & 0.21 &0.1923&0.4088&0.3964&0.3042 &0.4385& 0.3939&0.3168&0.3831\\

% \hspace{0.2cm} \textbf{\_compiled} & 0.5533 & 0.4911 & 0.3979 & 0.5198 &0.5188 & 0.412 &0.3314 &0.249  & 0.2032 &0.4151&0.4459 & 0.3532 &0.4549&0.4262&0.3416&0.4076\\

% \textbf{Coarse-grained} & 0.5277 & 0.5002 & 0.384 & 0.5708 & 0.5886& 0.4695 &0.344 &0.2809  & 0.2293 &0.4629&0.46 & 0.3808&0.4764&0.4574&0.3659&0.4332\\

% \hspace{0.2cm} \textbf{\_compiled}  & 0.5479 & \underline{0.5205} & \underline{0.4144} & \textbf{0.646} & \textbf{0.6529}& \textbf{0.5165} &\textbf{0.413} &\textbf{0.3298}  & \textbf{0.2796} &\underline{0.5235} &\underline{0.5217}  & \underline{0.3976}&\underline{0.5326}&\underline{0.5062}&\underline{0.402}&\underline{0.4803}\\
% \textbf{Fine-grained} & \underline{0.5702} & 0.504 & 0.3892 & \underline{0.6286} & \underline{0.6402}& \underline{0.492}&\underline{0.3637} &\underline{0.3171}  & 0.2497 &0.4774 &0.4668  & 0.37&0.5100&0.4820&0.3752&0.4557\\
% % 222(no format refine) & 0.5523 & 0.4773 & 0.3672 & \textbf{0.6331} & \underline{0.6411}& \underline{0.4934}&0.3637 &0.3177  & 0.2503 &0.4777 &0.4673  & 0.3704\\
% % 222 + MIPRO& 0.551 & 0.5132 & 0.3984 & 0.4778 & 0.5074& 0.4097 &0.2324 &0.283 & 0.2343 &0.5258 &0.5131  & 0.3862&0.4468&0.4542&0.3571&0.4174\\
% \hspace{0.2cm} \textbf{\_compiled} & \textbf{0.6354} & \textbf{0.5507} & \textbf{0.4389} & 0.6286 & 0.6402& 0.492 &0.3564&0.3166  & \underline{0.2671} &\textbf{0.5484} &\textbf{0.5325}  & \textbf{0.413}&\textbf{0.5422}&\textbf{0.51}&\textbf{0.4028}&\textbf{0.485}\\

% % \midrule
% % \midrule
% % \multicolumn{13}{l}{$\textbf{Compare results}$} \\
% % 222 + no explian& 0.5865 & 0.4949  & 0.383 & - & -& - &-&- & - &- &- & -\\

% % 222 + MIPRO(0-fewshot)& 0.5637 & 0.5101  & 0.3848 & 0.6211 & 0.635& 0.4877 &-&- & - &- &- & -\\

% % \midrule
% % \midrule
% % \multicolumn{13}{l}{$GPT3.5\_based\ baseline$} \\
% % G-eval & 0.4738 & 0.4522 & 0.3704 & 0.5835 &0.5902 & 0.4732 & - & - &- &~ & ~ & ~\\
% % % GPTScore-src & 0.4103 & 0.3618 & 0.2721 & 0.2497 & 0.2610& 0.1922 &- &-  & - \\
% % \midrule
% % \multicolumn{13}{l}{$\textbf{Ours\ GPT3.5\_based\ results}$}  \\
% % 111 &0.5825 &0.5413 & 0.4052  &0.5514 &0.5525  &0.4294 &- &-  & - &~ & ~ & ~\\
% % % 222 + MIPRO & 0.6682 & 0.5632 & 0.4205 & - & -& - &- &-  & - &~ & ~ & ~\\
% % 111 + fewshot & \textbf{0.6654} & 0.533 & 0.4138&\underline{0.6781 }&\underline{0.662}  & \underline{0.5241} &- &-  & - &~ & ~ & ~\\

% % 222\_multistage & 0.6424 & \underline{0.5931} & \underline{0.4441} & 0.6615 & 0.6615& 0.5002 &- &-  & - &~ & ~ & ~\\
% % % 222 + MIPRO & 0.6682 & 0.5632 & 0.4205 & - & -& - &- &-  & - &~ & ~ & ~\\
% % 222 + fewshot &\underline{0.6526} &\textbf{0.6109} & \textbf{0.48}& \textbf{0.7152} & \textbf{0.7289}& \textbf{0.558} &- &-  & - &~ & ~ & ~\\
% \bottomrule
% \end{tabular}
% }
% \caption{Main results based on Orca2-13B: Pearson ($\gamma$), Spearman ($\rho$) and Kendall-Tau ($\tau$) correlations between different metrics and human judgments of overall quality across four NLG evaluation tasks. We developed three experimental schemes: Vanilla, Coarse-grained, and Fine-grained, each including both a baseline experiment and an experiment with automated prompt optimization. In each column, the highest values are highlighted in \textbf{bold}, while the second-highest values are \underline{underlined}. 
% }
% \label{tab:main-result-orca2} 
% \end{table}
% % We reproduced other methods with a unified API
% % In main table, the name is not clear. 


% % [Figure 1.a]
% %  [Figure 1.b]
% %  [Figure 1.c]

==> tables/00_mian_gpt3.5.tex <==

% \begin{table}[htbp]
% \centering
% \begin{tabular}{lcccccc}
% \toprule
% ~ & \multicolumn{3}{c}{SummEval} & \multicolumn{3}{c}{TopicalChat} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7}  ~& $\gamma$ & $\rho$ & $\tau$ & $\gamma$ & $\rho$ & $\tau$ \\
% \midrule
% \multicolumn{7}{l}{$\textbf{Baseline\ (GPT-3.5-Based)}$} \\
% G-eval & 0.4738 & 0.4522 & 0.3704 & 0.5835 &0.5902 & 0.4732 \\
% % GPTScore-src & 0.4103 & 0.3618 & 0.2721 & 0.2497 & 0.2610& 0.1922 &- &-  & - \\
% \midrule
% \multicolumn{7}{l}{$\textbf{Our\ Results\ (GPT-3.5-Based)}$}  \\
% \textbf{SRE} (Coarse) & \textbf{0.6654} & 0.533 & 0.4138&\underline{0.6781 }&\underline{0.662}  & \underline{0.5241} \\
% % \hspace{0.2cm} -Unsupervised &0.5825 &0.5413 & 0.4052  &0.5514 &0.5525  &0.4294 \\
% % 222 + MIPRO & 0.6682 & 0.5632 & 0.4205 & - & -& - &- &-  & - &~ & ~ & ~\\
% \textbf{SRE} (Fine) &\underline{0.6526} &\textbf{0.6109} & \textbf{0.48}& \textbf{0.7152} & \textbf{0.7289}& \textbf{0.558} \\

% % \hspace{0.2cm} -Unsupervised & 0.6424 & \underline{0.5931} & \underline{0.4441} & 0.6615 & 0.6615& 0.5002 \\
% % 222 + MIPRO & 0.6682 & 0.5632 & 0.4205 & - & -& - &- &-  & - &~ & ~ & ~\\
% \bottomrule
% \end{tabular}
% \caption{Main results based on GPT-3.5: Pearson ($\gamma$), Spearman ($\rho$) and Kendall-Tau ($\tau$) correlations between different metrics and human judgments of overall quality on SummEval and TopicalChat. In each column, the highest values are highlighted in \textbf{bold}, while the second-highest values are \underline{underlined}. }
% \label{tab:main-result-gpt}
% \end{table}

% \begin{wraptable}{r}{0.6\textwidth} % 表格在右边，宽度为文档宽度的40%
% \centering
% \resizebox{0.6\textwidth}{!}{%
% \begin{tabular}{lcccccc}
% \toprule
% ~ & \multicolumn{3}{c}{SummEval} & \multicolumn{3}{c}{TopicalChat} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7}  ~& $\gamma$ & $\rho$ & $\tau$ & $\gamma$ & $\rho$ & $\tau$ \\
% \midrule
% G-eval & 0.4738 & 0.4522 & 0.3704 & 0.5835 &0.5902 & 0.4732 \\
% % GPTScore-src & 0.4103 & 0.3618 & 0.2721 & 0.2497 & 0.2610& 0.1922 &- &-  & - \\
% \midrule
% \multicolumn{7}{l}{$\textbf{Ours}$}  \\
% AC-Coarse & \textbf{0.6654} & 0.533 & 0.4138&\underline{0.6781 }&\underline{0.662}  & \underline{0.5241} \\
% % \hspace{0.2cm} -Unsupervised &0.5825 &0.5413 & 0.4052  &0.5514 &0.5525  &0.4294 \\
% % 222 + MIPRO & 0.6682 & 0.5632 & 0.4205 & - & -& - &- &-  & - &~ & ~ & ~\\
% AC-Fine &\underline{0.6526} &\textbf{0.6109} & \textbf{0.48}& \textbf{0.7152} & \textbf{0.7289}& \textbf{0.558} \\

% % \hspace{0.2cm} -Unsupervised & 0.6424 & \underline{0.5931} & \underline{0.4441} & 0.6615 & 0.6615& 0.5002 \\
% % 222 + MIPRO & 0.6682 & 0.5632 & 0.4205 & - & -& - &- &-  & - &~ & ~ & ~\\
% \bottomrule
% \end{tabular}
% }
% \caption{Main results based on GPT-3.5: Pearson ($\gamma$), Spearman ($\rho$) and Kendall-Tau ($\tau$) correlations between different metrics and human judgments of overall quality on SummEval and TopicalChat. In each column, the highest values are highlighted in \textbf{bold}, while the second-highest values are \underline{underlined}. }
% \label{tab:main-result-gpt}
% \end{wraptable}



\begin{wraptable}{r}{0.6\textwidth} % 表格在右边，宽度为文档宽度的40%
\centering
\vspace{-4mm}
\resizebox{0.55\textwidth}{!}{%
\begin{tabular}{lcccccc}
\toprule
~ & \multicolumn{3}{c}{SummEval} & \multicolumn{3}{c}{TopicalChat} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7}  ~& $\gamma$ & $\rho$ & $\tau$ & $\gamma$ & $\rho$ & $\tau$ \\
\midrule
G-eval & 0.4687 & 0.4504 & 0.3745 & 0.5427 &0.5597 & 0.4501 \\
% GPTScore-src & 0.4103 & 0.3618 & 0.2721 & 0.2497 & 0.2610& 0.1922 &- &-  & - \\
\midrule
\multicolumn{7}{l}{$\textbf{Ours}$}  \\
AC-Coarse & \textbf{0.6569} & \underline{0.5368} & \underline{0.4178}&\underline{0.6425 }&\underline{0.6171}  & \underline{0.4855} \\
% \hspace{0.2cm} -Unsupervised &0.5825 &0.5413 & 0.4052  &0.5514 &0.5525  &0.4294 \\
% 222 + MIPRO & 0.6682 & 0.5632 & 0.4205 & - & -& - &- &-  & - &~ & ~ & ~\\
AC-Fine &\underline{0.653} &\textbf{0.6016} & \textbf{0.4745}& \textbf{0.6718} & \textbf{0.6703}& \textbf{0.5156} \\

% \hspace{0.2cm} -Unsupervised & 0.6424 & \underline{0.5931} & \underline{0.4441} & 0.6615 & 0.6615& 0.5002 \\
% 222 + MIPRO & 0.6682 & 0.5632 & 0.4205 & - & -& - &- &-  & - &~ & ~ & ~\\
\bottomrule
\end{tabular}
}
\caption{Correlation between GPT-3.5-based evaluators and human judgments on instance-level overall quality for SummEval and TopicalChat. We compare Pearson ($\gamma$), Spearman ($\rho$) and Kendall-Tau ($\tau$) correlation, respectively. The best performance per indicator is highlighted in bold, and the second-highest results are underlined. We implemented and tested all the methods with p-value $<$ 0.05.%Main results based on GPT-3.5: Pearson ($\gamma$), Spearman ($\rho$) and Kendall-Tau ($\tau$) correlations between different metrics and human judgments of overall quality on SummEval and TopicalChat. In each column, the highest values are highlighted in \textbf{bold}, while the second-highest values are \underline{underlined}. 
}
\vspace{-5mm}
\label{tab:main-result-gpt}
\end{wraptable}

==> tables/01_Effectiveness_Explanation.tex <==
% \begin{table}[htp]
% \centering
% \begin{tabular}{ l c c c }
% \hline
% ~ & \textbf{$\gamma$} & \textbf{$\rho$} & \textbf{ $\tau$} \\ \hline
% Ours&0.5576&0.4975&0.4004\\
% $_{\_compiled}$&0.6165&0.5202&0.4153\\
% $_{\_w/o\ explanation}$ &0.541 &0.492  &0.3838\\
% $_{\_w/o\ inter}$ &0.5359 &0.4868  &0.3758\\

% \hline
% \end{tabular}
% \caption{Effectiveness of Explanation}\label{tab:04}
% \end{table}




\begin{table}[htp]
\centering
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
~& $\gamma$ & $\rho$ & $\tau$ &AVE\\
\midrule
\multicolumn{4}{l}{$Results\ with\ explanation (\textbf{Ours})$}  \\
Coarse-grained & 0.5077 & 0.5202 & 0.414  &0.4806\\

\hspace{0.2cm} \_compiled & 0.5479 & \underline{0.5205} & \underline{0.4144} &0.4943\\

Fine-grained & \underline{0.5702} & 0.504 & 0.3892 &0.4878 \\
\hspace{0.2cm} \_compiled & \textbf{0.6354} & \textbf{0.5507} & \textbf{0.4389} &0.5417\\

\hline
\multicolumn{4}{l}{${Results\ without\ explanation}$}  \\
Coarse-grained & 0.497 & 0.4981 & 0.3996  &0.4649\\

\hspace{0.2cm} \_compiled & 0.5453 & 0.5006 & 0.4091 &0.4850\\

Fine-grained & 0.5654 & 0.4889 & 0.3751  &0.4735\\
\hspace{0.2cm} \_compiled & 0.5568 & 0.4847 & 0.3998 &0.4804\\

\bottomrule
\end{tabular}
}
\caption{Effectiveness of Explanation. We report Pearson ($\gamma$), Spearman ($\rho$) and Kendall-Tau ($\tau$) correlations with and without explanation on SummEval.}
\label{tab:04}
\end{table}





\begin{table}[htp]
\centering
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
~& $\gamma$ & $\rho$ & $\tau$&AVE \\
\midrule
\multicolumn{4}{l}{$Results\ with\ explanation (\textbf{Ours})$}  \\
Coarse-grained & 0.5708 & 0.5886 & 0.4695  &0.5430\\

\hspace{0.2cm} \_compiled & 0.646 & 0.6529 & 0.5165 &0.6051\\

Fine-grained & 0.6286 & 0.6402 & 0.492 &0.5869 \\
\hspace{0.2cm} \_compiled & 0.6286 & 0.6402 & 0.492 &0.5869  \\

\hline
\multicolumn{4}{l}{${Results\ without\ explanation}$}  \\
Coarse-grained & 0.5681 & 0.5803 & 0.4595  &0.5363\\

\hspace{0.2cm} \_compiled & 0.6294& 0.6455 & 0.51&0.595 \\

Fine-grained & 0.5501 & 0.5736 & 0.4415  &0.5217\\
\hspace{0.2cm} \_compiled &0.5501 & 0.5736 & 0.4415 &0.5217 \\

\bottomrule
\end{tabular}
}
\caption{Effectiveness of Explanation. We report Pearson ($\gamma$), Spearman ($\rho$) and Kendall-Tau ($\tau$) correlations with and without explanation on Topical-chat.}
\label{tab:Topical-chat-Exp}
\end{table}




\begin{table}[htp]
\centering
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
~& $\gamma$ & $\rho$ & $\tau$&AVE \\
\midrule
\multicolumn{4}{l}{$Results\ with\ explanation (\textbf{Ours})$}  \\
Coarse-grained & 0.344 & 0.2809 & 0.2293  &0.2847\\

\hspace{0.2cm} \_compiled & 0.413 & 0.3298 & 0.2796 &0.3569\\

Fine-grained & 0.3637 & 0.3171 & 0.2497 & 0.3102\\
\hspace{0.2cm} \_compiled & 0.3564 & 0.3166 & 0.2671 & 0.3134 \\

\hline
\multicolumn{4}{l}{${Results\ without\ explanation}$}  \\
Coarse-grained & 0.3312 & 0.277 & 0.2148  & 0.2743\\

\hspace{0.2cm} \_compiled  & 0.3691& 0.3048 & 0.2701& 0.3147\\

Fine-grained & 0.3098 & 0.2743 & 0.2211  &0.2684\\
\hspace{0.2cm} \_compiled &0.3055 & 0.2864 & 0.2379 &0.2766 \\

\bottomrule
\end{tabular}
}
\caption{Effectiveness of Explanation. We report Pearson ($\gamma$), Spearman ($\rho$) and Kendall-Tau ($\tau$) correlations with and without explanation on sfres.}
\label{tab:sfres-Exp}
\end{table}




\begin{table}[htp]
\centering
\resizebox{0.47\textwidth}{!}{
\begin{tabular}{lcccc}
\toprule
~& $\gamma$ & $\rho$ & $\tau$&AVE \\
\midrule
\multicolumn{4}{l}{$Results\ with\ explanation (\textbf{Ours})$}  \\
Coarse-grained & 0.4629 & 0.46& 0.3808  &0.4346\\

\hspace{0.2cm} \_compiled & 0.5235 & 0.5217 & 0.3976 &0.4809\\

Fine-grained & 0.4774 & 0.4668 & 0.37 & 0.4381\\
\hspace{0.2cm} \_compiled & 0.5484 & 0.5325 & 0.413 &  0.498\\

\hline
\multicolumn{4}{l}{${Results\ without\ explanation}$}  \\
Coarse-grained & 0.4622 & 0.4536 & 0.342  &0.4193\\

\hspace{0.2cm} \_compiled & 0.4811& 0.4787 & 0.3799& 0.4466\\

Fine-grained & 0.4033 & 0.3948& 0.3051 &0.3677\\
\hspace{0.2cm} \_compiled &0.4697 & 0.4401 & 0.3809 & 0.4302\\

\bottomrule
\end{tabular}
}
\caption{Effectiveness of Explanation. We report Pearson ($\gamma$), Spearman ($\rho$) and Kendall-Tau ($\tau$) correlations with and without explanation on OPENMAVE.}
\label{tab: OPENMAVE-Exp}
\end{table}

==> tables/06_Explanation_visualization.tex <==


\begin{table}[htp]
  \centering
  \begin{tabular}{>{\raggedright\arraybackslash}p{15cm}}
\toprule
% \textbf{Response} \\
% \hline
% Paul merson has restarted his row with andros townsend . The tottenham midfielder was brought on with only seven minutes remaining in his team 's 0-0 draw with burnley . Andros townsend scores england 's equaliser in their 1-1 friendly draw with italy in turin .\\
% \hline
% \textbf{Score of Each Criterion} \\
% \hline
% Accuracy(0-100): The summary should accurately reflect the facts and details of the original text.
%  Score: 80,
 
% Completeness(0-100): All critical information and main ideas from the original text should be covered in the summary.
%  Score: 60,
 
% Conciseness(0-100): The summary should be brief, eliminating unnecessary details while retaining essential information.
%  Score: 70,
 
% Coherence(0-100): The summary should be logically structured and easy to follow.
%  Score: 50,
 
% Fluency(0-100): The language used in the summary should be smooth and natural.
%  Score: 70,
 
% Objectivity(0-100): The summary should be unbiased and present information without personal opinion unless required by the context.
%  Score: 80,
 
% Relevance(0-100): The content included in the summary should be relevant to the main focus of the original text.
%  Score: 90,
 
% Clarity(0-100): The summary should be clear and understandable without ambiguity.
%  Score: 70,
 
% Style(0-100): The writing style of the summary should be consistent and appropriate for the intended audience.
%  Score: 60,
 
% Grammatical Accuracy(0-100): The summary should be free from grammatical, spelling, and punctuation errors.
%  Score: 80,\\
% \hline
\textbf{Explaniation of Each}\\
\hline
\{

  "Coherence": \{
    "explanation": "The response logically presents the main events and details in a clear and cohesive manner, with a logical flow from one point to the next.",
    "score": 90 \},
  
  "Conciseness": \{
    "explanation": "The summary efficiently conveys all necessary information in a succinct manner without unnecessary verbosity.",
    "score": 85\},
    
  "Coverage": \{
    "explanation": "The summary captures the main events and details from the source text without omitting crucial information, providing a comprehensive overview of the situation.",
    "score": 95
  \},
  
  "Accuracy": \{
    "explanation": "The summary accurately reflects the main points and details of the source text, faithfully representing the key events and reactions.",
    "score": 90
  \},
  
  "Fluency": \{
    "explanation": "The language used in the summary is smooth and natural, with clear transitions between ideas and paragraphs, enhancing readability.",
    "score": 85
  \},
  
  "Relevance": \{
    "explanation": "The summary includes only pertinent information from the source text, maintaining relevance to the main topic and events.",
    "score": 95
  \},
  
  "Clarity": \{
    "explanation": "The summary is clear and comprehensible, using precise language to convey the main points and reactions effectively.",
    "score": 90
  \},
  
  "Engagement": \{
    "explanation": "The summary effectively captivates and engages the reader, drawing them into the main events and details with compelling language.",
    "score": 85
  \}
  
\}\\
\hline
\textbf{Explaniation of Overall}\\
\hline
The response provides a coherent and concise summary of the source text, covering the main events and details accurately and with relevance. The language used is clear and fluent, with good readability and natural transitions between ideas. However, the response could be more engaging to draw the reader into the main events and details more effectively.\\

\hline
\textbf{Score of Overall}\\
\hline
90.0\\
\bottomrule
  \end{tabular}
\caption{Explanation visualization} \label{tab:06}
\end{table}







==> tables/a1_Explanation_human_eval.tex <==



\begin{table}[ht]
\centering
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{|c|ccccc|c|c|c|}
\hline
\textbf{ID} & \textbf{Dimension} & \textbf{Clarity} & \textbf{Relevance} & \textbf{Score Alignment} & \textbf{Accuracy}&\textbf{Overall Alignment} & \textbf{Score Segment Differentiation} & \textbf{Overall} \\ \hline
\multirow{9}{1.5cm}{Instance (0-50)
} & Coherence & Yes / No & Yes / No & Yes / No& Yes / No & \multirow{9}{1.5cm}{Yes / No} & \multirow{9}{1.5cm}{Yes / No} & \multirow{9}{1.5cm}{1-5} \\ 
 & Conciseness & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Coverage & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Accuracy & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Fluency & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Relevance & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Clarity & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Engagement & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Overall Quality & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 \hline
\multirow{9}{1.4cm}{Instance (51-80)} & Coherence & Yes / No & Yes / No & Yes / No& Yes / No & \multirow{9}{1.5cm}{Yes / No} & \multirow{9}{1.5cm}{Yes / No} & \multirow{9}{1.5cm}{1-5} \\ 
 & Conciseness & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Coverage & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Accuracy & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Fluency & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Relevance & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Clarity & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Engagement & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Overall Quality & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 % \cline{1-6}
 \hline
\multirow{9}{1.4cm}{Instance (81-100)} & Coherence & Yes / No & Yes / No & Yes / No& Yes / No & \multirow{9}{1.5cm}{Yes / No} & \multirow{9}{1.5cm}{Yes / No} & \multirow{9}{1.5cm}{1-5} \\ 
 & Conciseness & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Coverage & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Accuracy & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Fluency & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Relevance & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Clarity & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Engagement & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 & Overall Quality & Yes / No & Yes / No & Yes / No& Yes / No & & & \\ 
 \hline
\end{tabular}
}
\caption{Human Evaluation for Explanation. GlobalA: Alignment eval between overall and each explanation. GlobalB: Case Level Differentiation Analysis}
\label{table:evaluation}
\end{table}


==> tables/a1_total_table.tex <==
\begin{table}[htbp]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lcccccccccccc|c}
\toprule
~ & \multicolumn{3}{c}{SummEval} & \multicolumn{3}{c}{TopicalChat} & \multicolumn{3}{c}{SFRES} & \multicolumn{3}{c|}{OpenMEVA}& \multirow{2}{*}{Average}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}  ~& $\gamma$ & $\rho$ & $\tau$ & $\gamma$ & $\rho$ & $\tau$ & $\gamma$ & $\rho$ & $\tau$ & $\gamma$ & $\rho$ & $\tau$ \\
\midrule
Auto-J & 0.1345 & 0.1457 & 0.1149 & 0.4681 &0.459 & 0.3714 & 0.126 & 0.1022 &0.0809&0.3896&0.3704&0.3065 & 0.2523\\
UniEval & 0.5457 & 0.4914 & 0.3707 & 0.5133 & 0.5448& 0.4134 &0.2894 &0.2499 & 0.1877&0.4501&0.4408&0.3119 &0.3855 \\
GPTScore-src & 0.4043 & 0.3584 & 0.2696 & 0.2313 & 0.2437& 0.1792 &0.2062 &0.121  & 0.1132&0.2283&0.2265&0.1534& 0.2227\\
ExplainEval & 0.5647 & 0.4916 & 0.3999 & 0.5542 & 0.5512 & 0.4476 & 0.1993 & 0.1181 &0.0946 &0.4809&0.4695&0.358&0.3941\\
% TIGERScore & 0.4422 & 0.3681 & 0.3129 & - & -& - &- &-  & - &0.4766&0.4636&0.3533&-&-&-\\
\midrule
%\multicolumn{13}{l}{$\textbf{Our\ Results\ (Orca2-13B)}$} \\
\multicolumn{13}{l}{$\textbf{Ours}$} \\
%\textbf{AC} (Vanilla)
\textsc{AC-Vnilla}& \underline{0.5494} & 0.486 & 0.3964 & 0.4932 &0.4927 & 0.4055 &0.2322 &0.1712  & 0.1398 &0.4023&0.4245 & 0.3209 &0.3651\\
%\textbf{SRE} (Coarse) 
%\textbf{SRE} (Coarse) 
\textsc{AC-Coarse} & 0.5386 & \underline{0.5227} & \underline{0.4156} & \textbf{0.611} & \underline{0.6173}& \textbf{0.4845} &\textbf{0.3094} &\textbf{0.2663}  & \textbf{0.199} &\underline{0.4908} &\underline{0.4962}  & \underline{0.3622}&\underline{0.4293}\\

w/o (a)&   0.5197 & 0.5045  &  0.389 &   0.5789&0.5808&  0.4617  &  0.2306 & 0.1896& 0.1342  &  0.4345 &0.4279&0.3461\\
w/o (b)&   0.51  & 0.4896 & 0.3846  &   0.5462  & 0.5509 &0.4182&  0.2096 &0.1611 &0.0902 &  0.3996&0.3812&0.3025  \\

% \textbf{SRE} (Fine) 
\textsc{AC-Fine} & \textbf{0.6301} & \textbf{0.5486} & \textbf{0.4299} & \underline{0.6023} & \textbf{0.6214}& \underline{0.4713} &\underline{0.3179}&\underline{0.2381}  & \underline{0.1985} &\textbf{0.5259} &\textbf{0.5363}  & \textbf{0.4109}&\textbf{0.4469}\\

w/o (a)&  0.5668 & 0.4993& 0.361 &  0.6023&0.6214&0.4713 & 0.2585 & 0.2194 &0.1741&0.4615&0.4518&0.374   \\
w/o (b)&  0.5589& 0.4873 & 0.3562 &  0.57&0.5671&0.4516&0.2146&0.1857&0.1523 &0.4168&0.41&0.3425 \\







\bottomrule
\end{tabular}
}
\caption{Correlation between LLM-based unified evaluators and human judgments on overall quality per instance across four NLG tasks. All train-free evaluators are built upon Orca2-13B. We compare Pearson ($\gamma$), Spearman ($\rho$) and Kendall-Tau ($\tau$) correlation, respectively. The best performance per indicator is highlighted in bold, and the second-highest results are underlined. %Main results based on Orca2-13B: Pearson ($\gamma$), Spearman ($\rho$) and Kendall-Tau ($\tau$) correlations between different metrics and human judgments of overall quality across four NLG evaluation tasks. We developed three experimental variants: Vanilla, Coarse-grained, and Fine-grained. We systematically investigated the performance variations of each variant under different optimization configurations. In each column, the highest values are highlighted in \textbf{bold}, while the second-highest values are \underline{underlined}. 
}
\label{tab:main-result-orca2} 
\end{table}


==> tables/b1.tex <==

\begin{table}[htp]
\centering
\resizebox{0.95\textwidth}{!}{%
\begin{tabular}{lcccccccccccc|ccc|c}
\toprule
~ & \multicolumn{3}{c}{SummEval} & \multicolumn{3}{c}{TopicalChat} & \multicolumn{3}{c}{SFRES} & \multicolumn{3}{c}{openMEVA}& \multicolumn{4}{c}{Average}\\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-17} ~& $\gamma$ & $\rho$ & $\tau$ & $\gamma$ & $\rho$ & $\tau$ & $\gamma$ & $\rho$ & $\tau$ & $\gamma$ & $\rho$ & $\tau$ & $\gamma$ & $\rho$ & $\tau$& AVE\\
\midrule
% \multicolumn{13}{l}{$Criterion\_based\ baseline\ Orca2-13b\_based$}  \\
% G-eval & 0.4649 & 0.4374 & 0.378 & 0.5075 & 0.4712 & 0.3802 &0.2642 & 0.2666 & 0.2060 &0.4158 &0.4262  & 0.3007 \\
% GPTScore & 0.2828 & 0.3105 & 0.2260 & \color{red}{0.0932} & \color{red}{0.0883} & \color{red}{0.0735} & 0.2712 & 0.2442 & 0.1837&-&-&- \\
% \midrule
\multicolumn{13}{l}{$Explanation\_based\ baseline\ Orca2-13b\_based$}  \\
IUST & 0.5746 & 0.5037 & 0.4038 & 0.5788 & 0.5706 & 0.4646 & 0.3068 & 0.2300 &0.1842 &0.4702&0.4611&0.3531&0.4826&0.4414&0.3539&0.4260\\
\midrule
\multicolumn{13}{l}{$Universal\ baseline$}  \\
auto-j & 0.1348 & 0.1464 & 0.1155 & 0.4819 &0.475 & 0.3927 & 0.1315 & 0.1053 &0.0869&0.3915&0.3799&0.3101 &0.2849&0.2767&0.2263&0.2626 \\
UniEval & 0.5569 & 0.4739 & 0.3780 & 0.5326 & 0.5769& 0.4363 &0.3247 &0.2791  & 0.2081&0.4488&0.4446&0.3122 & 0.4658& 0.4436&0.3337&0.4144\\
GPTScore-src & 0.4103 & 0.3618 & 0.2721 & 0.2497 & 0.2610& 0.1922 &0.2819 &0.2082  & 0.1618&0.2348&0.2319&0.1645&0.2942&0.2657&0.1977&0.2525 \\
% TIGERScore & 0.4422 & 0.3681 & 0.3129 & - & -& - &- &-  & - &0.4766&0.4636&0.3533&-&-&-\\
\midrule
\multicolumn{13}{l}{$\textbf{Ours\ Orca2-13b\_based\ results}$} \\
000 & 0.5284 & 0.4602 & 0.3689 & 0.5203 &0.5191 & 0.4118 & 0.3566 & 0.29 &0.2423&0.4988&0.4664&0.3642 &0.4760& 0.4339&0.3468&0.4189\\
000 + MIPRO & 0.5631 & \underline{0.5347} & \underline{0.4312} & 0.565 & 0.5911& 0.4805 &0.3345 &0.2716  & 0.2296 &0.5374 &0.506& 0.4072 &0.500&0.4759&0.3871&0.4543\\
000 + fewshot & 0.5533 & 0.4911 & 0.3979 & 0.5198 &0.5188 & 0.412 &0.3314 &0.249  & 0.2032 &0.4151&0.4459 & 0.3532 &0.4549&0.4262&0.3416&0.4076\\

111 & 0.5077 & 0.5202 & 0.414 & 0.5708 & 0.5886& 0.4695 &0.344 &0.2809  & 0.2293 &\textbf{0.5492}&\textbf{0.5408} & \underline{0.4228}&0.4929&0.4826&0.3839&0.4531\\
111 + MIPRO & 0.5839 & 0.5341 & 0.4222 & \underline{0.6304} & \underline{0.649}& \textbf{0.5191} &0.3799 &0.31 & 0.2513 &0.4771 &0.4748  & 0.3771&0.5178&0.4920&0.3924&0.4674\\
111 + few-shot & 0.5479 & 0.5205 & 0.4144 & \textbf{0.646} & \textbf{0.6529}& 0.5165 &\textbf{0.413} &\textbf{0.3298}  & \textbf{0.2796} &\underline{0.5412} &\underline{0.5233}  & \textbf{0.4248}&\textbf{0.5370}&\underline{0.5066}&\textbf{0.4088}&\textbf{0.4842}\\
222 & \underline{0.5702} & 0.504 & 0.3892 & 0.6286 & 0.6402& 0.492 &\underline{0.3637} &\underline{0.3171}  & 0.2497 &0.4774 &0.4668  & 0.37&0.5100&0.4820&0.3752&0.4557\\
% 222(no format refine) & 0.5523 & 0.4773 & 0.3672 & \textbf{0.6331} & \underline{0.6411}& \underline{0.4934}&0.3637 &0.3177  & 0.2503 &0.4777 &0.4673  & 0.3704\\
222 + MIPRO& 0.551 & 0.5132 & 0.3984 & 0.4778 & 0.5074& 0.4097 &0.2324 &0.283 & 0.2343 &0.5258 &0.5131  & 0.3862&0.4468&0.4542&0.3571&0.4174\\
222 + few-shot & \textbf{0.6354} & \textbf{0.5507} & \textbf{0.4389} & 0.6286 & 0.6402& 0.492 &0.3064&0.3166  & \underline{0.2671} &0.5265 &0.5294  & 0.3999&\underline{0.5242}&\textbf{0.5092}&\underline{0.3995}&\underline{0.4776}\\

% \midrule
% \midrule
% \multicolumn{13}{l}{$\textbf{Compare results}$} \\
% 222 + no explian& 0.5865 & 0.4949  & 0.383 & - & -& - &-&- & - &- &- & -\\

% 222 + MIPRO(0-fewshot)& 0.5637 & 0.5101  & 0.3848 & 0.6211 & 0.635& 0.4877 &-&- & - &- &- & -\\

\midrule
\midrule
\multicolumn{13}{l}{$GPT3.5\_based\ baseline$} \\
G-eval & 0.4738 & 0.4522 & 0.3704 & 0.5835 &0.5902 & 0.4732 & - & - &- &~ & ~ & ~\\
GPTScore-src & 0.4103 & 0.3618 & 0.2721 & 0.2497 & 0.2610& 0.1922 &- &-  & - \\
\midrule
\multicolumn{13}{l}{$\textbf{Ours\ GPT3.5\_based\ results}$}  \\
111 &0.5825 &0.5413 & 0.4052  &0.5514 &0.5525  &0.4294 &- &-  & - &~ & ~ & ~\\
% 222 + MIPRO & 0.6682 & 0.5632 & 0.4205 & - & -& - &- &-  & - &~ & ~ & ~\\
111 + fewshot & \textbf{0.6654} & 0.533 & 0.4138&\underline{0.6781 }&\underline{0.662}  & \underline{0.5241} &- &-  & - &~ & ~ & ~\\

222\_multistage & 0.6424 & \underline{0.5931} & \underline{0.4441} & 0.6615 & 0.6615& 0.5002 &- &-  & - &~ & ~ & ~\\
% 222 + MIPRO & 0.6682 & 0.5632 & 0.4205 & - & -& - &- &-  & - &~ & ~ & ~\\
222 + fewshot &\underline{0.6526} &\textbf{0.6109} & \textbf{0.48}& \textbf{0.7152} & \textbf{0.7289}& \textbf{0.558} &- &-  & - &~ & ~ & ~\\
\bottomrule
\end{tabular}
}
\caption{Correlation of LLM-based unified NLG evaluators with human judgments.}
\label{tab:00}
\end{table}



% \begin{table*}[ht]
% \centering
% \resizebox{0.95\textwidth}{!}{%
% \begin{tabular}{|c|cccc|c|c|c|}
% \hline
% \textbf{ID} & \textbf{Dimension} & \textbf{Consistency Rating} & \textbf{Error Detection} & \textbf{Usefulness Rating} & \textbf{GlobalA} & \textbf{GlobalB} & \textbf{Overall} \\ \hline
% \multirow{9}{*}{Case 1(0-35)
% } & Coherence & Yes / No & Yes / No & 1-5 & \multirow{9}{*}{Yes / No} & \multirow{27}{*}{Yes / No} & \multirow{27}{*}{1-5} \\ 
%  & Conciseness & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Coverage & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Accuracy & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Fluency & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Relevance & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Clarity & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Engagement & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Overall Quality & Yes / No & Yes / No & 1-5 & & & \\ \cline{1-6}
% \multirow{9}{*}{Case 2} & Coherence & Yes / No & Yes / No & 1-5 & \multirow{9}{*}{Yes / No} & &\\ 
%  & Conciseness & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Coverage & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Accuracy & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Fluency & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Relevance & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Clarity & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Engagement & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Overall Quality & Yes / No & Yes / No & 1-5 & & & \\ \cline{1-6}
% \multirow{9}{*}{Case 3} & Coherence & Yes / No & Yes / No & 1-5 & \multirow{9}{*}{Yes / No} & & \\ 
%  & Conciseness & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Coverage & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Accuracy & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Fluency & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Relevance & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Clarity & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Engagement & Yes / No & Yes / No & 1-5 & & & \\ 
%  & Overall Quality & Yes / No & Yes / No & 1-5 & & & \\ 
%  \hline
% \end{tabular}
% }
% \caption{Human Evaluation Table}
% \label{table:evaluation}
% \end{table*}





